Quantum neural networks

This PhD thesis combines two of the most exciting research areas of the last decades: quantum computing and machine learning. We introduce dissipative quantum neural networks (DQNNs), which are designed for fully quantum learning tasks, are capable of universal quantum computation and have low memory requirements while training. These networks are optimised with training data pairs in form of input and desired output states and therefore can be used for characterising unknown or untrusted quantum devices. We not only demonstrate the generalisation behaviour of DQNNs using classical simulations, but also implement them successfully on actual quantum computers. To understand the ultimate limits for such quantum machine learning methods, we discuss the quantum no free lunch theorem, which describes a bound on the probability that a quantum device, which can be modelled as a unitary process and is optimised with quantum examples, gives an incorrect output for a random input. Moreover we expand the area of applications of DQNNs in two directions. In the first case, we include additional information beyond just the training data pairs: since quantum devices are always structured, the resulting data is always structured as well. We modify the DQNN's training algorithm such that knowledge about the graph-structure of the training data pairs is included in the training process and show that this can lead to better generalisation behaviour. Both the original DQNN and the DQNN including graph structure are trained with data pairs in order to characterise an underlying relation. However, in the second extension of the algorithm we aim to learn characteristics of a set of quantum states in order to extend it to quantum states which have similar properties. Therefore we build a generative adversarial model where two DQNNs, called the generator and discriminator, are trained in a competitive way.

==> text/declaration.tex <==
\vspace*{\fill} 
\thispagestyle{empty}
\section*{Declaration}
Herewith, I, Kerstin Beer, born on 17.08.1993 in Hanover, declare that this thesis has been composed by myself and that it has not been submitted, in whole or in part, in any previous application for a degree. All sources and auxiliary materials used by me in this thesis are cited completely. I further declare that I agree to an examination following the faculty's regulations. I have not provided any direct or indirect monetary benefits to third parties for developing the content of this thesis. I agree that the dissertation will be checked for compliance with generally applicable scientific standards. 


\vspace{1.5cm}
\hspace{1 cm} Signature: \hspace{6cm} Date:

\vspace*{\fill} 
\addcontentsline{toc}{section}{Declaration}
